Physically interacting humans regulate muscle coactivation to improve visuo-haptic perception

When moving a piano or dancing tango with a partner, how should I control my arm muscles to best feel their movements and follow or guide them smoothly? Here we observe how physically connected pairs tracking a moving target with the arm modify muscle coactivation with their visual acuity and the partners performance. They coactivate muscles to stiffen the arm when the partners performance is worse, and relax with blurry visual feedback. Computational modelling show that this adaptive sensing property cannot be explained by movement error minimization proposed in earlier models. Instead, individuals skilfully control the arms stiffness to guide it on the planned motion while minimizing effort and extracting useful haptic information from the partners movement. The central nervous system regulates muscles' activation to guide motion with accurate task information from vision and haptics while minimizing the metabolic cost.

==> inputs/analysis.tex <==
The present study investigated effects of sensory feedback on a dyadic task in a within-subject design.
Three independent variables introduced in the study are the quality of the Visual feedback, Haptic feedback, and Epoch of trials. The Visual feedback relates to the own performance displayed on a computer screen which was either clean or noisy. Haptic feedback was controlled by means of the visual feedback to the dyadic partner which was also either clean or noisy. We call it haptic feedback as the visual feedback was not accessible and only experienced as haptic feedback from the perspective of the ``main" participant. We employed a full-factorial design, resulting in 4 experimental conditions; Clean(own)-Clean(other) or CC, Clean-Noisy~(CN), Noisy-Clean~(NC), Noisy-Noisy~(NN) for the first and second epoch each. These conditions were administered in a random order with a block 10 trials. In addition, the participants performed a block of 5 trials without a dyadic partner before (Solo1) and after (Solo2) the main experiment in order to facilitate task familiarization as well as to obtain their performance base-line. Thus, the experiment consists of $50$ trials that each lasted for~$20\ \mathrm{s}$. The last independent variable is Trial in which the first half and the second half of dependent variables were averaged into epochs in order to evaluate the short-term adaptation of performance within each experimental condition. 

The dependent variables are the tracking error and the cocontraction of the forearm estimated from the EMG measurements, averaged across the first and the second epochs of trials. The cocontraction data were organised to adhere to the experimental design from the ``own" perspective per participant, although the trials were performed in dyad. The statistical analysis on the cocontraction was performed using a three-way (Visual vs. Haptic vs. Trial) repeated-measures ANOVA. Due to the strong haptic couple of the devices used by the dyads, the tracking errors within a dyad were strongly correlated ($r(20) = .95, p<.0005$). Therefore, the tracking error was quantified per dyad (\textit{i.e.} $N=22$) instead of participant (\textit{i.e.} $N=44$) by taking their average. As a consequence, the mixed feedback conditions (CN and NC) becomes practically identical. Thus, all trials from CN and NC of the dyad were pooled together before averaging per epoch, resulting in three noise conditions; Clean, Mixed, Noisy. The effect of sensory noise on the tracking error was then analyzed in a two-way (Noise level vs Trial phase) repeated-measures ANOVA. An alpha level of .05 was used to quote statistical significance, and the Bonferroni correction was used for all subsequent multiple-comparisons.

==> inputs/data_processing.tex <==
\subsection{Joint kinematics and torque}
The joint angle and torque data were filtered by a fifth order Savitzky-Golay polynomial filter with a cut-off frequency of $10\ \mathrm{Hz}$.

The tracking error was calculated as 
\be
    e \equiv \, \left(\!\frac{1}{T} \! \int_0^T \!\!\! \left[q^*\!(t) - q(t) \right]^2 dt \!\right)^\frac{1}{2} \!\!,\, \,\,\, T \equiv 20\,s
\ee
, where $q(t)$ is the angle of the wrist.

In order to assess participants' tracking performance, the root mean squared of their kinematic error $\theta_{\mathrm{t}}-\theta_{\mathrm{w}}$ as

\begin{align}
	\mathrm{RMSE} = \sqrt{\frac{1}{n}\sum^{n}_{i=1}\left(\theta_{\mathrm{t},i}-\theta_{\mathrm{w},i}\right)^{2}}\ ,
	\label{eq:target}
\end{align}
, where $n$ is the total number of data points within the trial.

\subsection{EMG processing and cocontraction computation}
For each participant, muscle activities related to wrist flexion/extension muscle were collected from the flexor carpi radialis (FCR) and extensor carpi radialis longus (ECRL) using a medically certified non-invasive surface electromyography system (g.LADYBird + g.GAMMABox + g.BSamp, g.Tec) at 1000\,Hz. The EMG data were rectified and then low-pass filtered at 10\,Hz using a bidirectional second-order Butterworth filter to obtain the linear envelope. In order to isolate the EMG signals to flexion/extension muscle activation from passive muscle activation, the measurements from FCR and ECRL were truncated to zero when the joint torque value was negative and positive, respectively. The EMG data were then down-sampled to 100\,Hz to temporally align the joint angle and torque measurements for a normalization purpose. 

EMG normalization was performed for each participant prior to the study in order to map the raw muscle activity measured in millivolts to a corresponding torque value. The subject placed their wrist in the most comfortable middle posture, which was set to 0$^\circ$. Constrained at that posture, they were then instructed to sequentially {(\it i}) flex, or extend the wrist to exert a torque, or {(\it ii}) maximally co-contract in order to keep the wrist position stable during a 3\,Hz sinusoidal positional disturbance of 10$^\circ$ amplitude. Each phase was 4\,s long with a 5\,s rest period between consecutive contraction phases to avoid fatigue, which was used as a reference activity in the relaxed condition. This was repeated four times at flexion/extension torque levels \{1,2,3,4\}\,Nm and \{-1,-2,-3,-4\}\,Nm, respectively. For each subject, the recorded muscle activity was linearly regressed against the torque values to estimate the relationship between them. The torque of the flexor muscle was modelled as

\begin{equation}
    \begin{aligned}
        \tau_f(t) = \, \alpha_0 \, u_f(t) \, + \, \alpha_1 \,, \quad \alpha_0, \alpha_1 > 0 \,.
    \end{aligned}
    \label{eq:regression}
\end{equation}
Similarly for the extensor muscle torque $\tau_e$. \textit{Muscle cocontraction} was computed as

\begin{equation}
    \begin{aligned}
        u(t) \equiv \, \textup{min}\{\tau_f(t),\tau_e(t)\}\, .
    \end{aligned}
    \label{eq:cocon}
\end{equation}
%The normalized EMG signals were filtered by a fifth order Savitzky-Golay polynomial filter with a cut-off frequency of $10\ \mathrm{Hz}$.\issue{[this filter process is probably better removed. SE to re-process and check]} 

Based on the normalised EMG measurements, the reciprocal activation and the coactivation are calculated as 
\begin{align}
	a_{\mathrm{r}} &= a_{\mathrm{FCR}} + a_{\mathrm{ECRL}}\ ,\\
	a_{\mathrm{c}} &= \min\left(|a_{\mathrm{FCR}}|,|a_{\mathrm{ECRL}}|\right)\ ,
\end{align}
where $a_{\mathrm{r}}$ is the reciprocal activation, $a_{\mathrm{c}}$ is the coactivation, and $a_{\mathrm{FCR}}$ and $a_{\mathrm{ECRL}}$ are the torque-calibrated muscle activations of the FCR and ECRL muscles, respectively.

In order to be able to average and analyze these relative within-subject differences of the EMG data, we then normalize the reciprocal activation $a_{\mathrm{r}}$ and the coactivation $a_{\mathrm{c}}$ for each participant:
\begin{align*}
	\overline{a}_{\mathrm{r}} &= a_{\mathrm{r}}/a_{\mathrm{r,max}}\ ,\\
	\overline{a}_{\mathrm{c}} &= a_{\mathrm{c}}/a_{\mathrm{c,max}}\ ,
\end{align*}
where $\overline{a}_{\mathrm{r}}$ is the normalized reciprocal activation and $\overline{a}_{\mathrm{c}}$ is the normalized coactivation. The normalizing values $a_{\mathrm{r,max}}$ and $a_{\mathrm{c,max}}$ are given by the maximum values of the respective variables, averaged over time within trials. In order to exclude adaptation processes that occur during the first halves of the trials, the averages are calculated based on the second halves of the trials. 

\begin{figure}[ht]
	\includegraphics[width=1\columnwidth]{Figures/time_coact_norm_10s_ink.eps}
	\caption{\label{f:emg_time} Mean results of the coactivation $\overline{a}_{\mathrm{c}}$, averaged over trials within conditions and participants (solo: 5 trials, interaction: 10 trials). Note that there is a quick adaptation of co-contraction levels in the first half of a trial, and the EMG signals of the second half were used for data analyses.}
\end{figure}

==> inputs/protocol.tex <==
A participant was seated next to one of the interfaces, and instructed to place his/her right forearm on the interface and grasp the concavely shaped handle with his/her right hand. The forearm and the fingers were restrained by elastic straps in order to limit all possible movements to those of the wrist. The EMG electrodes were positioned on the FCR and ECRL muscles and tested for proper functionality. The participants were presented with examples of the visual feedback scenarios, and were informed of the resulting possible combinations. Each participant was asked to move his/her wrist to his/her most comfortable position in order to initialize the encoders and the torque sensors. After completion of these preparations, the curtain was drawn between the participants and they were instructed to not communicate verbally. The EMG calibration routine was performed and after its completion, the experiment was started. Verbal cues were provided by the experimenter, when the trial configuration changed from solo to interaction and vice versa. Visual cues were provided on the monitors, when the visual feedback scenarios changed between blocks of interaction trials. These visual cues indicated that a change would take place, but did not inform of the type of change.

The first 5 trials are solo trials, in which the participants perform the tracking task individually and do not experience any visual noise in their visual feedback. These trials allow for familiarization with the apparatus and simultaneously provide information on the individual behaviors of both participants. The following 40 trials are interaction~trials, in which the participants perform the tracking task while being physically coupled with the partner by a virtual spring. The last 5 trials are solo trials, which are identical to the first 5 trials. Participants were allowed to take small breaks avoid excessive fatigue during the course of the experiment.

==> inputs/results.tex <==
\subsection{Tracking performance}
The analysis on the tracking error indicates that the participants stabilized the task performance over the first five Solo trials as indicated by a reduction of the tracking error (2.35 $\pm$~0.51 degrees, 5th trial) in this condition to a similar magnitude during the last Solo trials~(2.24 $\pm$~0.59 degrees, 1st trial). Consistently, the tracking errors did not show any trend across trials in the dyadic conditions, as indicated by the lack of main effect on Trial phase by the two-way repeated-measures ANOVA, $p = .64$ On the other hand, the magnitude of the tracking error was gradually increased from when both interacting dyad receiving clean visual feedback~(1.88 $\pm$ 0.42 degrees), one of them receiving noisy feedback~(2.90 $\pm$ 0.53 degees), and both receiving noisy feedback~(2.25 $\pm$ 0.47 degrees). The main effect of Noise level is comfirmed by the ANOVA: $F(1,21) = 92.00, p<.0005$. A post-hoc comparion revealed that the significant differences between Clean and Mixed feedback~($p<.0005$), as well as Mixed and Noisy feedback~($p<.0005$). There was no interaction effect between Noise level and Trial phase ($p=.17$).

\begin{figure}[ht]
	\includegraphics[width=1\columnwidth]{Figures/angle.pdf}
	\caption{\label{f:results_error} The change in the tracking error across the experimental conditions. The error bars represent one standard error.}
\end{figure}

\subsection{Normalized cocontraction level}
Overall, there was a reduction of cocontraction level across trials, as supported by the 3-way repeated measures ANOVA,$F(1,43) = 53.58, p<.0005$, as is generally observed during learning \cite{Thoroughman1999, Franklin2008}, and is consistent with a slower adaptation of cocontraction level than motion and force \cite{Franklin2003}. The ANOVA also revealed the main effect of Visual noise, $F(1,43) = 85.91, p<.0005$, such that the cocontraction level reduced with the noise in the visual feedback (clean vs. noisy; 0.55 $\pm$  0.13 vs. 0.31 $\pm$ 0.18). In contrast, the noise in the haptic feedback increased the cocontraction level (clean vs. noisy; 0.40 $\pm$ 0.15 vs. 0.45 $\pm$ 0.14), and the ANOVA supports the observation, $F(1,43) = 7.33, p < .01$. The results contradict our hypothesis, as cocontraction was modulated in opposite way as observed in \cite{Carboni2020}. This inverted relationship was consistent with the statistical analysis indicated there was an interaction effect between the Visual and Haptic noises, $F(1,43) = 5.5257, p<.05$. Furthermore, there was also an interaction effect between Visual noise and Trial, $F(1,43) = 15.649, p <.0005$, indicating that the adaptation of the co-contraction level was significantly more prominent with respect to the Visual noise. Other interaction terms were not statistically significant ($p>.2$). 


\begin{figure}[ht]
	\includegraphics[width=1\columnwidth]{Figures/cocontraction.pdf}
	\caption{\label{f:results_emg} The change in the normalized cocontraction level across the experimental conditions. The error bars represent one standard error.}
\end{figure}

